Research on Third-Party Libraries in AndroidApps: A Taxonomy and Systematic LiteratureReview

Third-party libraries (TPLs) have been widely used in mobile apps, which play an essential part in the entire Android ecosystem. However, TPL is a double-edged sword. On the one hand, it can ease the development of mobile apps. On the other hand, it also brings security risks such as privacy leaks or increased attack surfaces (e.g., by introducing over-privileged permissions) to mobile apps. Although there are already many studies for characterizing third-party libraries, including automated detection, security and privacy analysis of TPLs, TPL attributes analysis, etc., what strikes us odd is that there is no systematic study to summarize those studies' endeavors. To this end, we conduct the first systematic literature review on Android TPL-related research. Following a well-defined systematic literature review protocol, we collected 74 primary research papers closely related to the Android third-party library from 2012 to 2020. After carefully examining these studies, we designed a taxonomy of TPL-related research studies and conducted a systematic study to summarize current solutions, limitations, challenges and possible implications of new research directions related to third-party library analysis. We hope that these contributions can give readers a clear overview of existing TPL-related studies and inspire them to go beyond the current status quo by advancing the discipline with innovative approaches.

==> Abstract.tex <==
\begin{abstract}
Third-party library (TPLs) is a double-edged sword. On the one hand, third-party libraries can facilitate the developing process of an app. On the other hand, they also bring various security risks, such as privacy leakage, over-privileged. Nowadays, there are many research work on third-party library from different perspectives, including third-party detection techniques, security and privacy analysis of TPLs, ad frauds studies, empirical studies, and exterior library analysis. What strikes us odd is that there is a lack of a systematic investigation for these state-of-the-art research. Little is known about the specific application scenarios of the current research on third-party libraries. Thus, in this paper, we aim at conducting a comprehensive and systematic investigation on current research of Android third-party library analysis. We first follow a well-defined systematic literature review methodology to collect 51 research papers regarding third-party analysis. Then we design a taxonomy for these papers based on different research purposes. We review their research background, core techniques, research purposes, the pros and cons. We also conduct a comparative study on existing research and provide an overview to readers from different perspectives. We hope that our work could give readers a clear understanding of TPLs analysis like a road-map in this direction.
\end{abstract}

% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
third-party library, Android, systematic investigation
\end{IEEEkeywords}


==> Background.tex <==
\section{Background}
\label{sec:preliminary}



%Android
\subsection{Third-party Library}
\label{sec:background:tpl}
If an app includes third-party libraries, the code mainly consists of two parts, the primary module from the host app and the supplementary (non-primary~\cite{PiggyApp13CODASPY}) module from third-party libraries.

Third-party libraries (TPLs) play an essential role in the development of apps development. TPLs enable efficient reuse of code possible. These TPLs are usually published as the ``.jar'' or ``.aar'' files. Considering various third-party libraries support powerful functionalities, developers can speed up their development progress by integrating TPLs into their apps. Besides, the reuse of high-quality TPL can also reduce the occurrence of error code.
Based on different functions, third-party libraries can be divided into different categories. AppBrain~\cite{AppBrain} roughly divides TPLs into three categories: Ad Networks, Social SDKs and developer tools. Prior research~\cite{Lin2014soups} divides TPLs into nine category. Based on the prior research, we divide the TPLs into types. The detailed classification is shown in the Table~\ref{tbl:libtype}.

\begin{table*}[thpb]
\centering
\caption{A taxonomy of Third-party library}
\begin{tabular}{lll}
\toprule
Category & Description & Examples  \\
\midrule
\rowcolor{gray!20}
Ad networks & A platform for ad companies to display in-app ads service & Admob,Inmobi \\
Content provider  & Provided by content provide to deliver relevant content, such as images or videos, etc.& Scribe\\
\rowcolor{gray!20}
Development aid & Help developing apps & Appyet, Novell \\
Game engine & Provide game framework for developers & Unity3d, Cocos2d\\
\rowcolor{gray!20}
Mobile analytics & Collect market analysis data for developers & Flurry, Umeng\\
Payment & Electronic payment service libs & Alipay,Mopay\\
\rowcolor{gray!20}
Social networking service & Embed social network services in mobile networks & Facebook,Twitter\\
Utility & Utility java libs & Jsoup, Nostra13  \\
\rowcolor{gray!20}
UI components & Provide customized UI components & Kankan,Decsmart\\

\bottomrule
\end{tabular}
\label{tbl:libtype}
\end{table*}


\begin{comment}


\subsection{Research on Third-party Library}
\label{sec:background:researchonTPL}
In sum, the existing research on third-party libraries (TPLs) can be divided into three parts: TPLs detection, interior lib analysis, and exterior lib analysis. We explain these different research directions in detail in the following subsection.


\subsubsection{Third-party Detection}
There are two main methods to identify third-party libraries. The first one is a whitelist-based approach and the second one is non-prior \todo{knowledge-based} method. The whitelist-based method uses the package name to identify third-party libraries. There are many disadvantages to this approach. The whitelist cannot contain the whole third-party libraries. It is difficult to find new libraries. Therefore, there is a hysteresis in this method. The whitelist-based method uses the package name to identify third-party libraries. A recent study showed that more than 50\% inspected Android third-party libs are protected by obfuscation techniques~\cite{Lin2014soups}. Therefore, this method is not resilient to package name-based obfuscation. Given the disadvantages as mentioned before, many research~\cite{AdDetect2014ISSNIP,PiggyApp13CODASPY,LibRadar2016ICSE,LibD2017ICSE} try to use the lib features to find third-party libraries. LibRadar~\cite{LibRadar2016ICSE} extracts the stable feature Android API as the code feature and hash the feature vector to represent the library package. LibD~\cite{LibD2017ICSE} does not completely depend on package structure. It employs the package structure as the auxiliary information. The authors first construct the control flow graph (CFG) and then extract the opcode in each block of CFG as the code feature. In sum, the research in this direction is promising.


\subsubsection{Interior Library Analysis}

Interior lib analysis mainly includes empirical study or analysis of some feature of TPLs, such as the UI features, traffic features or some special behaviors analysis. Some research\cite{ad2016NDSS,pluto2016,AdRisk2012Wisec} focus on the security vulnerability of third-party libraries. Some research~\cite{Most2012,price2016NDSS} attempt to find the privacy leakage of TPLs. Some work~\cite{FraudDroid2018FSE,MadFraud2014mobisys} research the ad fraud. Book et al.~\cite{MOST2013} analyzed the permission characteristics of ad libs. He et al.~\cite{MAdLens2018infocom}
summarized the UI features of ad libs. We will later discuss these work in the following section.


\subsubsection{Exterior Library Analysis}

The exterior analysis mainly focuses on the impact of libs on other analysis.
The prior research points out that the third-party code could account more than 60\% of the code in the Android apps on average. The code of TPLs is a non-negligible factor for app analysis because they introduce some noises and directly affect the accuracy of the detection result. In-app malware detection and repackaged app detection, many techniques have already attempted different methods to delete TPLs. MassVet~\cite{MassVet2015chen} employs a whitelist which includes 73 third-party libraries to remove TPLs. Wukong~\cite{Wukong2015issta} and PiggyApp~\cite{PiggyApp13CODASPY} use clustering-based method to filter out third-party libraries. Li et al.~\cite{Lili2016SANER} explain the impact of third-party libs in repackaging detection. CLANdroid~\cite{CLANDroid2016ICPC} verifies TPLs can affect the accuracy of results. Some work ~\cite{Mojia2014software,Gui2017WhatAO} study the impact of ad libs on app rating.


\end{comment}

==> Threats.tex <==
\section{Threats To Validity}
\label{sec:threats}

Even though we have attempted our best to collect related papers as many as possible by following the state-of-the-art SLR methodology, our search results may still miss some relevant papers. One reason may be that some existing repository search engines are not very accurate; they may provide some irrelevant papers. The other reason may be that our keywords cannot find all the relevant papers. 

==> category.tex <==
 \section{Review of TPL Research}
\label{sec:review}

In this section, we mainly introduce TPLs related research based on the Taxonomy in section~\ref{sec:Taxonomy}.

%################################################
%\subsection{Third-party Libraries Isolation}









%Zhan et al.~\cite{splitads2017ACISP} extended the current permission mechanism, which can let the developers configure permission policy at the library level. LibCage~\cite{Libcage2016ESORICS} and SanAdBox~\cite{sanAdBox2013ICC} proposed a sandbox for third-party libraries to achieve the privilege separation.
%PEDAL~\cite{PEDAL2015MobiSys} sets up three different resource access rules of TPLs and rewrites the core resources assess and sharing functions of bytecode to achieve the privilege de-escalation.
%Aframe~\cite{aframe2013ACSAC} isolates the untrusted TPLs into a different process with a different UID from the main app. It achieves the process isolation, permission isolation, and input/output isolation.
%AdDroid~\cite{AdDroid20120ASISCCS} introduces new advertising permissions to protect the API and implement the privilege separation. We will give more detailed comparison information in section~\ref{sec:comparison}.


%###################################################################

%\subsection{TPLs Detection}



%################


\subsection{Empirical Studies}







==> name.tex <==
%We find that all of these existing detection tool have four common disadvantages:

%\textbf{1) require collect a large set of input at construction stage.} Whether it is clustering-based method or similarity-based method, they need to developers or researchers collect a large set of Android apps or TPL version files. LibRadar uses 1 million Android apps to construct their TPL database. The entire pre-construction phase is very time-consuming and labor-intensive. It requires a lot of effort to replicate the whole project.

%\textbf{ 2) hard to find newly-emerging and niche TPLs.} The pre-defined database is difficult to find an arbitrary library in an app. Given the clustering-based method, it easily omits some uncommon-used TPLs. To ensure the recall, similarity comparison method requires developers to collect a large number of TPL files. LibScout only collect 164 TPL with 2065 versions in their database, this magnitude is far from enough for real world TPL detection. Therefore, the biggest problem of existing database-driven approach is that the recall usually not very high. Based on our experiment in Section~\ref{sec:evaluation:RQ1}, the recall of all of these publicly-available tools do not exceed 50\%. The highest recall comes from LibScout, only reached 49.03\%. Note that the TPLs in the ground truth even does not cover all TPLs used in the app in our dataset. Excluding the apps are obfuscated by package renaming technique, there are still more than 94,00 TPLs in our app set. LibScout detected the largest number of TPLs, but only reached 1335 which accounts for 14\% of the total TPLs. Not to mention other TPL detection tools. Based on the above data, we can find that the biggest problem of existing detection tool is low detection coverage rate.

%\textbf{3) module decoupling is not considered.} To us surprise, all of these publicly-available tools do not consider module decoupling, and all tools are take the code of host app into account, which lead to cost extra computing resources. Wang et al.~\cite{Wang2017ICSE-C,Wukong2015issta} pointed out that more than 60\% of the code in an Android app are TPLs, which means the code of the host app accounts for about 40\%. These parts of code will cost extra computing resources. Besides, not excluding the host app can also cause other problems. Given the clustering-based method, it assumes that when inputting a large set of apps, the TPLs would be clustered into big groups because the same libraries are used by many different apps~\cite{Wukong2015issta}. If we do not exclude the primary module (the code from the host app), this assumption may bring some problem. This assumption omits the repackaged apps and some apps developed by the template. If the set includes groups repackaged apps\footnote{the repackaged apps only consider the code of host apps are similar}, these signatures of repackage apps will be added into the database. To some extend, it might slow down the search speed. LibSift~\cite{LibSift2016soh} employs the module decoupling method to identify the primary module and split the TPLs, but it does not conduct the library identification. Besides, LibSift just leverages the package name that is extracted from the \texttt{AndroidManifest.xml} file  to delete the primary module. Based on our research, we find that many activities in the primary module may have different name with the package name. This situation mostly comes from repackaged apps or some game apps. We analyzed more than 20,000 apps and find more than a half of apps have this situation. For example, there is an app named ``com.housepaint.game'', we do find some components belong to this package but even the Main Activity belongs to another different package ``com.unity3d.player''. In addtion, this assumption also omits the repackaged apps and apps obfuscated by package flatten technique. Therefore, the method used by LibSift to identify the primary module will cause many false positives.

%\textbf{4) pre-setting assumptions are too strong to affect the detection performance.}

%\xian{Furthermore, we also find some disadvantages of each TPL detection tool. LibRadar and ORLIS do not consider the new feature when the Android apps are construct on API level 21 or higher versions. The detection rate of LibRadar and ORLIS will sharply decrease when they handle apps with multiple Dex files (Section~\ref{sec:evaluation:RQ2}).}

